Understanding the Effect of Algorithm Transparency of Model Explanations in Text-to-SQL Semantic Parsing

Explaining the decisions of AI has become vital for fostering appropriate user trust in these systems. This paper investigates explanations for a structured prediction task called ``text-to-SQL Semantic Parsing'', which translates a natural language question into a structured query language (SQL) program. In this task setting, we designed three levels of model explanation, each exposing a different amount of the model's decision-making details (called ``algorithm transparency''), and investigated how different model explanations could potentially yield different impacts on the user experience. Our study with $\sim$100 participants shows that (1) the low-/high-transparency explanations often lead to less/more user reliance on the model decisions, whereas the medium-transparency explanations strike a good balance. We also show that (2) only the medium-transparency participant group was able to engage further in the interaction and exhibit increasing performance over time, and that (3) they showed the least changes in trust before and after the study.

==> discussion-conclusion.tex <==
\section{Discussion}

\zyc{Ziyu will add: (1) how can AI and HCI researchers collaborate? -> automatic metric as surrogate, or human-in-the-loop explanation design. (2) human-AI collaboration, considering further factors such as the expert cost in explanation design.}


\subsection{Designing More Effective Explanations for Users} 
Explanations for AI predictions should help users determine when and when not to trust the AI's prediction, particularly in high-stakes applications where errors can be costly and issues of safety and bias are critical. If explanations can reliably signal when to trust or challenge AI predictions, AI adoption in various domains could be safer, even if the models aren't always accurate. However, a key issue identified in our study, consistent with previous findings, is that current explanations tend to persuade participants to accept AI predictions without sufficient scrutiny. We conjecture that this may be due to explanations primarily focusing on justifying the AI’s output, rather than critically evaluating it. Therefore, we argue that developing explanation methods that help users especially identify incorrect AI predictions is essential. For example, to verify an AI's response to a query (e.g., "List the names of professors in the CS department above age 56"), a human participant or another AI model could generate follow-up or counterfactual questions (e.g., "List the names of CS professors" or "List the names and ages of CS professors") and provide their AI-generated answers, enabling users to cross-check the consistency of the responses.

Additionally, we observed that providing too much or too little explanation about the AI's decision-making process leads to a decline in overall accuracy and participants' engagement with the explanations over time. This emphasizes the importance of balancing the cognitive load of participants by providing just enough information for participants to evaluate AI predictions effectively. Thus, a more effective strategy may involve an interactive approach, where explanations are provided incrementally based on participants' needs, rather than overwhelming them with extensive details upfront. In addition, the explanations can also be optimized to make them more engaging by including different visual aids and interactive elements.

\subsection{Trust-calibration using the explanations of varying levels of transparency}
Human user trust is a key factor in determining when they decide to rely on or not rely on an AI’s predictions. Over-trust can result in users blindly accepting AI outputs, while under-trust can cause excessive skepticism. The goal is to foster appropriate trust, where users accept the AI's predictions when they are correct and remain cautious when the predictions are incorrect. TBD


\section{Conclusion}

